SplatFormer: Point Transformer for Robust 3D Gaussian Splatting

3D Gaussian Splatting (3DGS) has recently transformed photorealistic reconstruction, achieving high visual fidelity and real-time performance. However, rendering quality significantly deteriorates when test views deviate from the camera angles used during training, posing a major challenge for applications in immersive free-viewpoint rendering and navigation. In this work, we conduct a comprehensive evaluation of 3DGS and related novel view synthesis methods under out-of-distribution (OOD) test camera scenarios. By creating diverse test cases with synthetic and real-world datasets, we demonstrate that most existing methods, including those incorporating various regularization techniques and data-driven priors, struggle to generalize effectively to OOD views. To address this limitation, we introduce SplatFormer, the first point transformer model specifically designed to operate on Gaussian splats. SplatFormer takes as input an initial 3DGS set optimized under limited training views and refines it in a single forward pass, effectively removing potential artifacts in OOD test views. To our knowledge, this is the first successful application of point transformers directly on 3DGS sets, surpassing the limitations of previous multi-scene training methods, which could handle only a restricted number of input views during inference. Our model significantly improves rendering quality under extreme novel views, achieving state-of-the-art performance in these challenging scenarios and outperforming various 3DGS regularization techniques, multi-scene models tailored for sparse view synthesis, and diffusion-based frameworks.

==> Figures_tex/supp_results-mvimgnet.deprecated.tex <==
\begin{figure}[t!]
    % \vspace{-1em}
    \centering
    \scriptsize 
    \setlength{\tabcolsep}{0.0mm} 
    \newcommand{\sz}{0.16}
    \newcommand{\szi}{0.12}
    \newcommand{\szh}{0.2}
    \renewcommand{\arraystretch}{0.0}
    % \newcommand{\compareexamplerow}[1]{
    %         \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet_mehr/#1_cam} &
    %     \includegraphics[width=\szi\linewidth,]{Figures/results_mvimgnet_mehr/#1_gs} &
    %         \includegraphics[width=\szi\linewidth]{Figures/results_mvimgnet_mehr/#1_pred} &
    %         \includegraphics[width=\szi\linewidth]{Figures/results_mvimgnet_mehr/#1_gt} \\
    % } 
    \newcommand{\compareexamplerow}[1]{
            \includegraphics[height=\szh\linewidth]{Figures/results_mvimgnet_mehr/#1_cam} &
        \includegraphics[height=\szh\linewidth,,trim={0 3cm 0 0},clip]{Figures/results_mvimgnet_mehr/#1_gs} &
            \includegraphics[height=\szh\linewidth,trim={0 3cm 0 0},clip]{Figures/results_mvimgnet_mehr/#1_pred} &
            \includegraphics[height=\szh\linewidth,trim={0 3cm 0 0},clip]{Figures/results_mvimgnet_mehr/#1_gt} \\
    } 
    
    \begin{tabular}{cccc}  % 8 images
           %  \compareexamplerow{11_12}
           %  \compareexamplerow{15_11}
           Camera Setup&3DGS&Ours&GT \\
            \compareexamplerow{33_4}
            \compareexamplerow{35_1}
            \compareexamplerow{43_13}
            \compareexamplerow{59_14}
            \compareexamplerow{29_14}
    \end{tabular}
    \caption{\textbf{The potential of SplatFormer in handling in-the-wild, unbounded scenes.} When trained on MVImgNet (in-the-wild unbounded scenes), SplatFormer learns to partially remove floaters, though refining objects' flawed geometry remains a challenge.} 
    \label{fig:supp_mvimgnet}
\end{figure}

% \begin{figure}[t!]
%     % \vspace{-1em}
%     \centering
%     \scriptsize 
%     \setlength{\tabcolsep}{0.0mm} 
%     \newcommand{\sz}{0.17}
%     \renewcommand{\arraystretch}{0.0}
%     \begin{tabular}{cccc}  % 8 images
%            Camera Setup&3DGS&Ours&GT \\
% \phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
%             \includegraphics[width=0.25\linewidth]{Figures/results_mvimgnet/0_cameras.pdf} &
%             \hspace{1mm}
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/0_pred_highlight} &
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/0_ours_highlight} &
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/0_gt}
%             \\
% \phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
%             Camera Setup&3DGS&Ours&GT \\
% \phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
%             \includegraphics[width=0.25\linewidth]{Figures/results_mvimgnet/6_cameras.pdf} &
%             \hspace{1mm}
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/6_pred} &
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/6_ours} &
%             \includegraphics[width=\sz\linewidth]{Figures/results_mvimgnet/6_gt}
%             \\
%     \end{tabular}
%     \caption{\textbf{The potential of SplatFormer in handling in-the-wild, unbounded scenes.} When trained on MVImgNet (in-the-wild unbounded scenes), SplatFormer learns to partially remove floaters, though refining objects' flawed geometry remains a challenge.} 
%     \label{fig:supp_mvimgnet}
% \end{figure}


==> Figures_tex/supp_results-objaverse.bkup.tex <==
\begin{figure}[t!]
    % \vspace{-1em}
    \centering
    \scriptsize % Sets the text within the figure to a smaller font size.
    \setlength{\tabcolsep}{0mm} %0 Adjusts the spacing between columns in the table. A small value creates tightly packed columns.
    \newcommand{\sz}{0.120}  % 0.33 Defines a new command \sz to represent a size fraction (16% of the linewidth). This size is used later to control image sizes.
    \renewcommand{\arraystretch}{0} %Reduces the vertical space between rows in the table to near zero, making rows more compact.
    % Define a new command that compares one example across multiple methods
    \newcommand{\compareexamplerow}[1]{
            \begin{tabular}{ccccccc}
            Four of Inputs&\text{MipNeRF360}&\text{Nerfbusters}&\text{InstantNGP}&\text{SyncDreamer}&\text{LaRa}&\text{SSDNeRF} \\
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_gt_2x2} &\hspace{1mm}
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_mipnerf360} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_nerfbusters} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_instantngp} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_syncdreamer} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_lara} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_ssdnerf} \\
            % \vspace{3mm}
% \phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
\text{GT}& \text{Ours}&\text{2DGS}&\text{SplatFields}&\text{FSGS}&\text{3DGS}& \text{InstantSplat} \\
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_gt} &\hspace{1mm}
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_ours} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_2dgs} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_splatfield} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_fsgs} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_3dgs} &
            \includegraphics[width=\sz\linewidth]{Figures/results/#1_instantsplat} \\
\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}&\phantom{+++}\\
            \end{tabular}
    } %Define a new command to include images with common formatting
\compareexamplerow{2f8e8e42522c418e8e5f35b2d7e55eab-20-test_elevation80_step2}
\compareexamplerow{8fafbb7ee0714802add43db11debb5c1-20-test_elevation90_step0}
% \compareexamplerow{914d43018c9b4cd681e31d56cb889563-10-test_elevation90_step1} red car
% \compareexamplerow{3e66059c275548c4a183b2f9e085f953-10-test_elevation90_step2} %plane as failure case
\compareexamplerow{5fcd426a7d754a95b64ea21f34b762ea-10-test_elevation80_step2}
\compareexamplerow{3e288ee8aced4a0797e66d53536112b1-10-test_elevation80_step2}
% \compareexamplerow{0af0dfc6afd045d9990aa688f6c792ff-20-test_elevation70_step1}
% \compareexamplerow{0a6e1a80d2e34d5981d6b2b440bbc8cd-10-test_elevation90_step1} blue jet
\compareexamplerow{29d27ef9f80145f1ad5a166952d04557-20-test_elevation80_step2}
% \compareexamplerow{5fcd426a7d754a95b64ea21f34b762ea-10-test_elevation80_step2}
% \compareexamplerow{81fe61e043ba411c951e4b3b80e82ca4-20-test_elevation80_step2}

% \compareexamplerow{3a64ef3f2e8a4b4f9d3ebdb835053df9-20-test_elevation90_step2}

    \caption{\textbf{Results on Objaverse-OOD.} We compare our method with baselines: SyncDreamer~\citep{liu2023syncdreamer}, LaRa~\citep{LaRa}, SSDNeRF~\citep{ssdnerf}, 3DGS~\citep{kerbl3dgs}, Nerfbusters~\citep{Nerfbusters2023}, SplatFields~\citep{SplatFields}, InstantSplat~\cite{fan2024instantsplat}, 2DGS~\citep{huang20242dSplat_Tuebingen}, FSGS~\citep{zhu2023FSGS_texas}, InstantNGP~\citep{mueller2022instantngp}, and MipNeRF360~\citep{barron2022mipnerf360}.} 
    \label{fig:exp_full_objaverse}
\end{figure}

% %In main text:
% \input{figures_tex/exp_static_recon}


==> tables_tex/supp_efficiency.tex <==
\begin{wraptable}[7]{r}{7.0cm} % [19]
    \scriptsize
    \setlength{\tabcolsep}{0.6pt}
    \vspace{-2em}
    \caption{\textbf{Memory Usage and Inference Time.}} \label{tab:supp_efficiency}
 \resizebox{7.0cm}{!}{
    \begin{tabular}[t]{c|ccc|c}
    \toprule
      Number of Splats & 10k–40k & 60k–70k & 90k-100k & Average \\
    \midrule
      Memory (MB)&675&801&1010&782\\
      Time (ms)&62&70&118&75\\
    \bottomrule
    \end{tabular}
}
\end{wraptable}
